Rank Also Matters: Hierarchical Configuration for Mixture of Adapter Experts in LLM Fine-Tuning

Large language models (LLMs) have demonstrated remarkable success across various tasks, accompanied by a continuous increase in their parameter size. Parameter-efficient fine-tuning (PEFT) methods, such as Low-Rank Adaptation (LoRA), address the challenges of fine-tuning LLMs by significantly reducing the number of trainable parameters. Recent studies have integrated LoRA with Mixture of Experts (MoE) architectures, leveraging multiple adapter experts and gating mechanisms to further improve fine-tuning performance. However, existing approaches primarily focus on adjusting the allocations of adapter experts per layer to optimize the introduced trainable parameter size, while neglecting a critical factor of adapters' rank. To this end, we propose a hierarchical scheme for expert allocation and rank configuration, HILO, which dynamically adjusts the number and rank of adapter experts across layers, matching the varying representational complexity of model layers in adapter-granularity. Extensive experiments on multiple benchmark tasks demonstrate that HILO outperforms existing methods in accuracy while introducing fewer trainable parameters, providing an efficient and practical solution for fine-tuning LLMs.

==> table.tex <==
% \begin{table*}[t]
% \centering
%     \begin{tabular}{lcccccccccccc}
%     \toprule
%     & \multicolumn{3}{c}{Adapter Expert Setting} & \multicolumn{2}{c}{Parameter $\downarrow$} & \multicolumn{6}{c}{Accuracy (\%) $\uparrow$} \\
%     \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-13}
%     \multirow{-2}{*}{Method}& {Exp.} & {Rank} & {Top-$K$} & {Active} & {Trainable} & {SQA} & {CQA} & {OQA} & {MRPC} & {COLA}  & {RET} & {Avg.}\\
%     \midrule
%     Llama\,2 & - & - & - & - & - & 40.23 & 20.58 & 25.20 & 66.55 & 55.99  & 53.42 & 43.66\\
%     \midrule
%     Vanilla  & 8  & 8  & 2 & 2 & 1 & 90.10 & 78.21 & 76.20 & 85.15 & 84.85  & 87.72 & 83.71\\
%     \midrule
%     MoLA & $\triangledown$ & 8 & 2 & 2 & 0.63 & 89.61 & \textbf{76.00} & 74.20 & 84.23 & 85.52  & 84.47 & 82.34\\
%     \rowcolor{gray!15}{\name} & 8  & $\triangledown$ & 2 & \textbf{1.25} & 0.63 & \textbf{90.42} & 75.92 & \textbf{76.20} & \textbf{84.52} & \textbf{86.19} & \textbf{84.48} & \textbf{82.96}\\
%     \midrule
%     AlphLoRA & $ \ddagger$ & 8 & 2 & 2 & 0.63 & 89.70 & 75.83 & 74.60 & 82.49 & 85.13 & 85.55 & 82.22\\
%     \rowcolor{gray!15}\name & $\ddagger\ddagger$ & $\triangledown$ & 2 & \textbf{1.25} & 0.63 & \textbf{90.15} & \textbf{76.58} & \textbf{75.80} & \textbf{84.46} & \textbf{84.27} & \textbf{88.09} & \textbf{83.23}\\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparison of methods with different setting. \fcolorbox{white}{gray!15}{\name Ours}}\label{tab:method_comparison1}
% \end{table*}

% % \begin{table*}[t]
% %     \centering
% %     \caption{Top-2}\label{tab:transposed_table}
% %     \begin{tabular}{lccccccccc}
% %     \toprule
% %     & \multicolumn{2}{c}{Parameter $\downarrow$} & \multicolumn{7}{c}{Accuracy (\%) $\uparrow$}\\
% %     \cmidrule(lr){2-3} \cmidrule(lr){4-10}
% %     \multirow{-2}{*}{Method} & Active & Trainable & SQA & CQA & OQA & MRPC & COLA & RET & Avg. \\
% %     \midrule
% %     MoLA & 2 & 1 & 89.61 & 76.00 & 74.20 & 84.23 & 85.52 & 84.47 & - \\
% %     \rowcolor{gray!15} \name & 0.78 & 0.39 & 89.29 & 76.74 & 76.80 & 83.47 & 85.61 & 84.11 & - \\
% %     \bottomrule
% %     \end{tabular}
% % \end{table*}



% \begin{table}[t]
%     \centering
%     \begin{tabular}{lc>{\columncolor{gray!15}}cc>{\columncolor{gray!15}}c}
%     \toprule
%      & \multicolumn{2}{c}{Active Parameter $\downarrow$} & \multicolumn{2}{c}{Accuracy (\%) $\uparrow$}\\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%     \multirow{-2}{*}{Dataset} & AdaMoE & \name & AdaMoE & \name\\
%     \midrule
%     {SQA}  & 1.05 & \textbf{0.68} & 89.43 & \textbf{90.06}\\
%     {CQA}  & 1.01 & \textbf{0.63} & 75.26 & \textbf{75.43}\\
%     {OQA}  & 1.03 & \textbf{0.63} & 72.60 & \textbf{73.60}\\
%     {MRPC} & 1.03 & \textbf{0.64} & 84.81 & \textbf{85.62}\\
%     {COLA} & 1.01 & \textbf{0.63} & 85.42 & \textbf{85.81}\\
%     {RET}  & 1.09 & \textbf{0.67} & 81.94 & \textbf{85.20}\\
%     \midrule
%     {Avg.} & 1.04 & \textbf{0.65} & 81.58 & \textbf{82.62}\\
%     \bottomrule
%     \end{tabular}
%     \caption{experts=8, null experts=8, rank=8/$\triangledown$,Top-2}\label{tab:my_label}
% \end{table}

% \begin{table}[t]
% \centering
%     \begin{tabular}{ccccc}
%     \toprule
%     \multicolumn{2}{c}{Adapter Experts} & \multicolumn{2}{c}{Parameter $\downarrow$} &  \\
%     \cmidrule(lr){1-2} \cmidrule(lr){3-4}
%     {Rank} & {Top-K} & {Active} & {Trainable} & \multirow{-2}{*}{{Accuracy (\%) $\uparrow$}} \\
%     \midrule
%     8 & 2 & 1.03 & 0.63 & 88.44 \\
%     \rowcolor{gray!15}$\triangledown$ & 2 & \textbf{0.77} & \textbf{0.39} & \textbf{89.74} \\
%     \midrule
%     8 & $\triangledown$ & 1.65 & 0.63 & \textbf{90.56} \\
%     \rowcolor{gray!15}$\triangledown$ & $\triangledown$ & \textbf{1.23} & \textbf{0.39} & 90.24 \\
%     \bottomrule
%     \end{tabular}
%     \caption{AdaMoE-Ablation experts=null experts=$\triangledown$ in SQA dataset}\label{tab:ablation_experiments}
% \end{table}
